VinVL: Revisiting Visual Representations in Vision-Language Models

This paper presents a detailed study of improving visual representations for vision language (VL) tasks and develops an improved object detection model to provide object-centric representations of images. Compared to the most widely used \emph{bottom-up and top-down} model \cite{anderson2018bottom}, the new model is bigger, better-designed for VL tasks, and pre-trained on much larger training corpora that combine multiple public annotated object detection datasets. Therefore, it can generate representations of a richer collection of visual objects and concepts. While previous VL research focuses mainly on improving the vision-language fusion model and leaves the object detection model improvement untouched, we show that visual features matter significantly in VL models. In our experiments we feed the visual features generated by the new object detection model into a Transformer-based VL fusion model \oscar \cite{li2020oscar}, and utilize an improved approach \short\ to pre-train the VL model and fine-tune it on a wide range of downstream VL tasks. Our results show that the new visual features significantly improve the performance across all VL tasks, creating new state-of-the-art results on seven public benchmarks. We will release the new object detection model to public.

==> subtex/tables.tex <==

\begin{table*}[h!]
\begin{center}
\scriptsize
\caption{Evaluation results on COCO dataset. (Note: \texttt{B} for Base, \texttt{L} for Large)}
\vspace{-0mm}
\label{tab:mscoco_retrieval}
\begin{tabular}{@{\hspace{0mm}}l@{\hspace{0mm}}c|@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}|c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{1mm}}|c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{1mm}}|c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{0mm}}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\texttt{Size}} & \multicolumn{3}{c|}{Text Retrieval} & \multicolumn{3}{c|}{Image Retrieval} & \multicolumn{3}{c|}{Text Retrieval} & \multicolumn{3}{c}{Image Retrieval}\\ 
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\ 
%\hline \hline
\midrule
& & \multicolumn{6}{c|}{1K Test Set} & \multicolumn{6}{c}{5K Test Set} \\ 
\hline
DVSA~\cite{karpathy2015deep} & - & $38.4$ & $69.9$ & $80.5$ & $27.4$ & $60.2$ & $74.8$ & - & - & - & - & - & -  \\
%m-CNN~\cite{ma2015multimodal} & - & $42.8$ & $73.1$ & $84.1$ & $32.6$ & $68.6$ & $82.8$ & $41.3$ & - & $81.2$ & $30.3$ & - & $72.4$ \\
%DSPE~\cite{wang2016learning} & - & $50.1$ & $79.7$ & $89.2$ & $39.6$ & $75.2$ & $86.9$ \\
VSE++~\cite{faghri2017vse++} & - & $64.7$ & - & $95.9$ & $52.0$ & - & $92.0$ & $41.3$ & - & $81.2$ & $30.3$ & - & $72.4$ \\
DPC~\cite{zheng2017dual} & - & $65.6$ & $89.8$ & $95.5$ & $47.1$ & $79.9$ & $90.0$ & $41.2$ & $70.5$ & $81.1$ & $25.3$ & $53.4$ & $66.4$ \\
CAMP~\cite{wang2019camp} & - & $72.3$ & $94.8$ & $98.3$  & $58.5$ & $87.9$  & $95.0$ & $50.1$ & $82.1$ & $89.7$  & $39.0$ & $68.9$  & $80.2$ \\
SCAN~\cite{lee2018stacked} & - & $72.7$ & $94.8$ & $98.4$ & $58.8$ & $88.4$ & $94.8$ & $50.4$ & $82.2$ & $90.0$ & $38.6$ & $69.3$ & $80.4$ \\ 
SCG~\cite{shi2019knowledge} & - & $76.6$ & $96.3$ & $99.2$ & $61.4$ & $88.9$ & $95.1$ & $56.6$ & $84.5$ & $92.0$ & $39.2$ & $68.0$ & $81.3$ \\
PFAN~\cite{wang2019position} & - & $76.5$ & $96.3$ & $99.0$ & $61.6$ & $89.6$ & $95.2$ & - & - & - & - & - & - \\
%Unicoder-VL (w/o pre-training) & \texttt{B} & $75.1$ & $94.3$ & $97.8$ & $63.9$ & $91.6$ & $96.5$ \\
Unicoder-VL~\cite{li2019unicoder} & \texttt{B} & $84.3$ & $97.3$ & $99.3$ & $69.7$ & $93.5$ & $97.2$ & $62.3$ & $87.1$ & $92.8$ & $46.7$ & $76.0$ & $85.3$ \\ 
12-in-1~\cite{lu201912} & \texttt{B} & - & - & - & $65.2$ & $91.0$ & $96.2$ & - & - & - & - & - & - \\ 
UNITER~\cite{chen2019uniter} & \texttt{B} & - & - & - & - & - & - & $63.3$ & $87.0$ & $93.1$ & $48.4$ & $76.7$ & $85.9$ \\
UNITER~\cite{chen2019uniter} & \texttt{L} & - & - & - & - & - & - & $66.6$ & $89.4$ & $94.3$ & $51.7$ & $78.4$ & $86.9$ \\ \hline
%ImageBERT~\cite{qi2020imagebert} & \texttt{B} & $85.4$ & $97.3$ & $99.8$ & $73.6$ & $94.3$ & $97.2$ \\ \hline
%\multirow{3}{*}{\short{}} & \texttt{B} & \textcolor{blue}{$\bf 87.5$} & \textcolor{blue}{$\bf 99.2$} & \textcolor{blue}{$\bf 99.7$} & \textcolor{blue}{$\bf 75.1$} & \textcolor{blue}{$\bf 95.1$} & \textcolor{blue}{$\bf 97.9$} \\ 
\multirow{2}{*}{\short{}} & \texttt{B} & \cellcolor{Gray}$88.4$ & \cellcolor{Gray}\textcolor{blue}{$\bf 99.1$} & \cellcolor{Gray}\textcolor{blue}{$\bf 99.8$} & \cellcolor{Gray}$75.7$ & \cellcolor{Gray}$95.2$ & \cellcolor{Gray}$98.3$ & \cellcolor{Gray}$70.0$ & \cellcolor{Gray}$91.1$ & \cellcolor{Gray}$95.5$ & \cellcolor{Gray}$54.0$ & \cellcolor{Gray}$80.8$ & \cellcolor{Gray}$88.5$ \\ %\hline
 & \texttt{L} & 
 \cellcolor{Gray}\textcolor{blue}{$\bf 89.8$} & \cellcolor{Gray}$ 98.8$ & \cellcolor{Gray}$99.7$ & 
 \cellcolor{Gray}\textcolor{blue}{$\bf 78.2$} & \cellcolor{Gray}\textcolor{blue}{$\bf 95.8$} & \cellcolor{Gray}\textcolor{blue}{$\bf 98.3$} & \cellcolor{Gray}\textcolor{blue}{$\bf 73.5$} & \cellcolor{Gray}\textcolor{blue}{$\bf 92.2$} & \cellcolor{Gray}\textcolor{blue}{$\bf 96.0$} & \cellcolor{Gray}\textcolor{blue}{$\bf 57.5$} & 
 \cellcolor{Gray} \textcolor{blue}{$\bf 82.8$} & 
 \cellcolor{Gray} \textcolor{blue}{$\bf 89.8$} \\
%\midrule
%\multicolumn{8}{c}{5K Test Set} \\ \hline
%VSE++~\cite{faghri2017vse++} & - & $41.3$ & - & $81.2$ & $30.3$ & - & $72.4$ \\
%DPC~\cite{zheng2017dual} & - & $41.2$ & $70.5$ & $81.1$ & $25.3$ & $53.4$ & $66.4$ \\
%CAMP~\cite{wang2019camp} & - & $50.1$ & $82.1$ & $89.7$  & $39.0$ & $68.9$  & $80.2$ \\
%SCAN~\cite{lee2018stacked} & - & $50.4$ & $82.2$ & $90.0$ & $38.6$ & $69.3$ & $80.4$ \\
%SCG~\cite{shi2019knowledge} & - & $56.6$ & $84.5$ & $92.0$ & $39.2$ & $68.0$ & $81.3$ \\
%Unicoder-VL~\cite{li2019unicoder} & \texttt{B} & $62.3$ & $87.1$ & $92.8$ & $46.7$ & $76.0$ & $85.3$ \\
%UNITER~\cite{chen2019uniter} & \texttt{B} & $63.3$ & $87.0$ & $93.1$ & $48.4$ & $76.7$ & $85.9$ \\
%UNITER~\cite{chen2019uniter} & \texttt{L} & $66.6$ & $89.4$ & $94.3$ & $51.7$ & $78.4$ & $86.9$ \\
%\hline
%\multirow{2}{*}{\short{}} & \texttt{B} & $70.0$ & $91.1$ & $95.5$ & $54.0$ & $80.8$ & $88.5$ \\ %\hline
% & \texttt{L} & \textcolor{blue}{$\bf 73.5$} & \textcolor{blue}{$\bf 92.2$} & \textcolor{blue}{$\bf 96.0$} & \textcolor{blue}{$\bf 57.5$} & \textcolor{blue}{$\bf 82.8$} & \textcolor{blue}{$\bf 89.8$} \\ 
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table*}




\begin{table*}[h!]
\begin{center}
\caption{Image captioning evaluation results (single model) on COCO "Karpathy" test split. (Note: B@4: BLUE@4, M: METEOR, C: CIDEr, S: SPICE.)}
\scriptsize
\label{tab:mscoco_caption}
\begin{tabular}{l@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c|}{cross-entropy optimization} & \multicolumn{4}{c}{CIDEr optimization}\\ 
& B@4 & M & C & S & B@4 & M & C & S\\ \midrule
BUTD~\cite{anderson2018bottom} & $36.2$ & $27.0$ & $113.5$ & $20.3$ & $36.3$ & $27.7$ & $120.1$ & $21.4$ \\
VLP~\cite{zhou2019unified} & $36.5$ & $28.4$ & $117.7$ & $21.3$ & $39.5$ & $29.3$ & $129.3$ & $23.2$ \\ 
AoANet~\cite{huang2019attention} & $37.2$ & $28.4$ & $119.8$ & $21.3$ & $38.9$ & $29.2$ & $129.8$ & $22.4$ \\ \hline
%\shortb{} & $36.4$ & $\bf 30.3$ & $\bf 123.4$ & $\bf 23.0$ & $\bf 41.5$ & $\bf 30.3$ & $\bf 137.6$ & $\bf 23.8$ \\
%{'Bleu_1': 0.7559008579599475, 'Bleu_2': 0.5996653451461248, 'Bleu_3': 0.46710442171328737, 'Bleu_4': 0.36391776678284776, 'METEOR': 0.30210555494130015, 'ROUGE_L': 0.5826219366204061, 'CIDEr': 1.2364127000822858, 'SPICE': 0.23128705106248199} application_1580189644036_10498/output/checkpoint-37-84000
\rowcolor{Gray} 
\shortb{} & $36.5$ & $\bf 30.3$ & $\bf 123.7$ & $\bf 23.1$ & $\bf 40.5$ & $\bf 29.7$ & $\bf 137.6$ & $\bf 22.8$ \\
%\shortb{} & $36.5$ & $\bf 30.3$ & $\bf 123.7$ & $\bf 23.1$ & $\bf 41.5$ & $\bf 30.3$ & $\bf 137.6$ & $\bf 23.8$ \\
%{'Bleu_1': 0.7573752359884675, 'Bleu_2': 0.6008378397373233, 'Bleu_3': 0.46787010774302273, 'Bleu_4': 0.3647869689751411, 'METEOR': 0.30265313409088807, 'ROUGE_L': 0.5839181967668083, 'CIDEr': 1.2371494497965225, 'SPICE': 0.2308596427512451} application_1580189644036_10498/output/checkpoint-39-88000
%\shortl{} & $36.8$ & \textcolor{blue}{$\bf 30.5$} & \textcolor{blue}{$\bf 126.0$} & \textcolor{blue}{$\bf 23.5$} & \textcolor{blue}{$\bf 42.1$} & \textcolor{blue}{$\bf 30.5$} & \textcolor{blue}{$\bf 140.5$} & \textcolor{blue}{$\bf 24.4$} \\
%\shortl{} & $36.8$ & \textcolor{blue}{$\bf 30.6$} & \textcolor{blue}{$\bf 126.7$} & \textcolor{blue}{$\bf 23.5$} & \textcolor{blue}{$\bf -$} & \textcolor{blue}{$\bf -$} & \textcolor{blue}{$\bf -$} & \textcolor{blue}{$\bf -$} \\ %application_1580189644036_9602/output/checkpoint-28-128000,
\rowcolor{Gray} 
%\shortl{} & \textcolor{blue}{$\bf 37.4$} & \textcolor{blue}{$\bf 30.7$} & \textcolor{blue}{$\bf 127.8$} & \textcolor{blue}{$\bf 23.5$} & \textcolor{blue}{$\bf 42.1$} & \textcolor{blue}{$\bf 30.5$} & \textcolor{blue}{$\bf 140.5$} & \textcolor{blue}{$\bf 24.4$} \\%ab70_img_large_cap_ce_ep7_816k/pt-results/application_1580189644036_9602/output/checkpoint-28-128000
\shortl{} & \textcolor{blue}{$\bf 37.4$} & \textcolor{blue}{$\bf 30.7$} & \textcolor{blue}{$\bf 127.8$} & \textcolor{blue}{$\bf 23.5$} & \textcolor{blue}{$\bf 41.7$} & \textcolor{blue}{$\bf 30.6$} & \textcolor{blue}{$\bf 140.0$} & \textcolor{blue}{$\bf 24.5$} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}




%For base model, we fine-tune the model for N epochs with a learning rate of 5e-5 and a batch size of 128. For large model, we fine-tune the model for 25 epochs with a learning rate of 3e-5 and a batch size of 96. 
%For inference, we add constrained beam search~\cite{}. 


\begin{table*}[h!]
\begin{center}
\caption{NoCaps val set. Models are trained on COCO only without pre-training.}
\scriptsize
\label{tab:nocaps_caption}
\begin{tabular}{l@{\hspace{2mm}}|c@{\hspace{1mm}}c@{\hspace{1mm}}|c@{\hspace{1mm}}c@{\hspace{1mm}}|c@{\hspace{1mm}}c@{\hspace{1mm}}|c@{\hspace{1mm}}c}
\toprule
\multirow{2}{*}{Method } & \multicolumn{2}{c|}{in-domain} & \multicolumn{2}{c|}{near-domain} & \multicolumn{2}{c|}{out-of-domain} & \multicolumn{2}{c}{overall}\\ 
& CIDEr & SPICE & CIDEr & SPICE & CIDEr & SPICE & CIDEr & SPICE \\ \midrule
 \multicolumn{9}{c}{Validation Set} \\ \hline
UpDown~\cite{agrawal2019nocaps} & $78.1$ & $11.6$ & $57.7$ & $10.3$ & $31.3$ & $8.3$ & $55.3$ & $10.1$ \\
UpDown + CBS~\cite{agrawal2019nocaps} & $80.0$ & $12.0$ & $73.6$ & $11.3$ & $66.4$ & $9.7$ & $73.1$ & $11.1$ \\
UpDown + ELMo + CBS~\cite{agrawal2019nocaps} & $79.3$ & \textcolor{blue}{$\bf 12.4$} & $73.8$ & $11.4$ & $71.7$ & $9.9$ & $74.3$ & $11.2$ \\
%UpDown+++~\cite{agrawal2019nocaps} & $84.2$ & $12.6$ & $82.1$ & $11.9$ & $86.7$ & $10.6$ & $83.3$ & $11.8$ \\
%Human~\cite{agrawal2019nocaps} & $84.4$ & $14.3$ & $85.0$ & $14.3$ & $95.7$ & $14.0$ & $87.1$ & $14.2$ \\ 
\midrule
%BERT & $68.0$ & $11.2$ & $51.4$ & $10.0$ & $29.2$ & $8.1$ & $49.3$ & $9.8$ \\ \midrule
%\multicolumn{9}{c}{without pre-training} \\ \hline
% BERT$_{B}$ & $68.9$ & $11.2$ & $51.5$ & $10.0$ & $27.3$ & $8.0$ & $49.1$ & $9.8$ \\ 
%BERT$_{B}$-{vg} & $75.9$ & $12.2$ & $60.5$ & $11.1$ & $36.7$ & $8.8$ & $57.9$ & $10.8$ \\ 
%%BERT$_{B}$-{vg} + SCST & $82.2$ & $11.9$ & $63.2$ & $11.0$ & $37.8$ & $9.0$ & $60.8$ & $10.8$ \\ 
%BERT$_{B}$-{vg} + CBS & $78.5$ & $12.2$ & $75.3$ & $11.8$ & $74.2$ & $10.3$ & $75.5$ & $11.6$ \\ 
%BERT$_{B}$-{vg} + SCST + CBS & $82.6$ & $11.9$ & $79.1$ & $11.9$ & $76.4$ & $10.4$ & $79.0$ & $11.6$ \\ 
\rowcolor{Gray} 
\shortb{} & $79.6$ & $12.3$ & $66.1$ & $11.5$ & $45.3$ & $9.7$ & $63.8$ & $11.2$ \\
%BERT$_{B}$-{oid} + SCST & $82.9$ & $11.9$ & $66.5$ & $11.1$ & $44.7$ & $9.6$ & $64.4$ & $10.9$ \\
\rowcolor{Gray} 
\shortb{} + CBS & $80.0$ & $12.1$ & $80.4$ & \textcolor{blue}{$\bf 12.2$} & $75.3$ & \textcolor{blue}{$\bf 10.6$} & $79.3$ & \textcolor{blue}{$\bf 11.9$} \\ 
\rowcolor{Gray} 
\shortb{} + SCST + CBS & $\bf 83.4$ & $12.0$ & $\bf 81.6$ & $12.0$ & $\bf 77.6$ & \textcolor{blue}{$\bf 10.6$} & $\bf 81.1$ & $11.7$ \\ 
\rowcolor{Gray}
\shortl{} & $79.9$ & \textcolor{blue}{$\bf 12.4$} & $68.2$ & $11.8$ & $45.1$ & $9.4$ & $65.2$ & $11.4$ \\
\rowcolor{Gray} 
\shortl{} + CBS & $78.8$ & $12.2$ & $78.9$ & $\bf 12.1$ & $77.4$ & $10.5$ & $78.6$ & $\bf 11.8$ \\ 
\rowcolor{Gray} 
\shortl{} + SCST + CBS & \textcolor{blue}{$\bf 85.4$} & $11.9$ & \textcolor{blue}{$\bf 84.0$} & $11.7$ & \textcolor{blue}{$\bf 80.3$} & $10.0$ & \textcolor{blue}{$\bf 83.4$} & $11.4$ \\ 
\midrule
\multicolumn{9}{c}{Test Set} \\ \hline
\rowcolor{Gray} 
\shortb{} + SCST + CBS & $81.3$ & $11.9$ & $79.6$ & \textcolor{blue}{$\bf 11.9$} & $73.6$ & \textcolor{blue}{$\bf 10.6$} & $78.8$ & \textcolor{blue}{$\bf 11.7$} \\ 
\rowcolor{Gray} 
\shortl{} + SCST + CBS & \textcolor{blue}{$\bf 84.8$} & \textcolor{blue}{$\bf 12.1$} & \textcolor{blue}{$\bf 82.1$} & $11.5$ & \textcolor{blue}{$\bf 73.8$} & $9.7$ & \textcolor{blue}{$\bf 80.9$} & $11.3$ \\ 
%\midrule
%\multicolumn{9}{c}{with pre-training} \\ \hline
%\textsc{Baseline (No Tags)} & $80.4$ & $12.3$ & $64.6$ & $11.3$ & $35.3$ & $8.9$ & $60.9$ & $11.0$ \\ \midrule
%\multicolumn{9}{c}{with \short{} pre-training} \\ \hline
%\shortb{}-{vg} & $82.7$ & $12.8$ & $68.8$ & $11.8$ & $41.9$ & $9.4$ & $65.4$ & $11.5$\\ 
%%\shortb{}-{vg} + SCST  & $91.4$ & $13.0$ & $74.1$ & $12.0$ & $47.3$ & $9.8$ & $71.2$ & $11.7$ \\
%\shortb{}-{vg} + SCST + CBS & $87.0$ & $12.6$ & $83.5$ & $12.4$ & $80.9$ & $11.0$ & $83.5$ & $12.1$ \\
%\shortl{}-{vg} + SCST + CBS & $88.9$ & $12.7$ & $84.5$ & $12.6$ & $81.2$ & $11.1$ & $\bf 84.5$ & $\bf 12.3$ \\
%\shortb{}-{oid} & $86.5$ & $13.0$ & $79.2$ & $12.5$ & $54.7$ & $10.3$ & $75.3$ & $12.2$\\ 
%\shortb{}-{oid} + SCST + CBS & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


\begin{table*}[h!]
\begin{center}
\caption{Evaluation results on VQA.}
\vspace{-0mm}
\scriptsize
\label{tab:vqa_result}
\begin{tabular}{l|ccccccc|>{\columncolor[gray]{0.90}}c>{\columncolor[gray]{0.90}}c}
\toprule
Method & ViLBERT & VL-BERT & VisualBERT & LXMERT & 12-in-1 & \textsc{UNITER}$_\text{B}$ & \textsc{UNITER}$_\text{L}$  & \shortb{} & \shortl{} \\ \midrule
%& B@4 & M & C & S & B@4 & M & C & S\\ \midrule
Test-dev & $70.63$ & $70.50$ & $70.80$ & $72.42$ & $73.15$ & $72.27$ & $\bf 73.24$ & $73.16$ & \textcolor{blue}{$\bf 73.61$} \\
Test-std & $70.92$ & $70.83$ & $71.00$ & $72.54$ & $-$ & $72.46$ & $73.40$ & $\bf 73.44$ & \textcolor{blue}{$\bf 73.82$} \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table*}

LXMERT improves the SoTA overall accuracy (‘Accu’ in Table 2) by 2.1\%. and has 2.4% improvement on the ‘Binary’/‘Other’ question sub-categories. Although LXMERT does not explicitly take a counting module as in BAN+Counter, our result on the counting-related questions (‘Number’) is still equal or better

\textbf{VQA} and \textbf{NLVR2} are the two major V+L understanding tasks widely used to evaluate the exsiting VLP models. 
Table~\ref{tab:vqa_result} summarizes the evaluation results on VQA task. We can see that \shortb{} is the best among the models with equivalent size, even slightly better than UNITER~\cite{chen2019uniter} large. And the \shortl{} creates new single-model SoTAs on VQA and NLVR2. As mentioned in Section~\ref{sec:NLVR2}, the NLVR2 fine-tuning architecture is still not the best choice, we believe there is still space to improve, we leave this for future exploration.


this is not necessarily  the best fine-tuning choice for NLVR2, please refer to the \textit{Pair-biattn} finetuning in UNITER~\cite{chen2019uniter} for better choice, which introduces a multi-head attention layer to look back the concatenated text-image sequences.

One of major understanding tasks for the exsiting VLP models is VQA. From Table~\ref{tab:vqa_result}, we can see that \shortb{} is the best among the models with equivalent size, even slightly better than UNITER~\cite{chen2019uniter} large. 



And the \shortl{} creates new single-model SoTAs on VQA and NLVR2. 

\begin{table*}[t!]
\begin{center}
\caption{Evaluation results on NLVR2.}
\scriptsize
\vspace{-0mm}
\label{tab:nlvr2_result}
\begin{tabular}{l|cccccc|>{\columncolor[gray]{0.90}}c>{\columncolor[gray]{0.90}}c}
\toprule
Method & MAC & VisualBERT & LXMERT & 12-in-1 & \textsc{UNITER}$_\text{B}$ & \textsc{UNITER}$_\text{L}$ & \shortb{} & \shortl{} \\ \midrule
%Dev & $50.8$ & $67.40$ & $74.90$ & $-$ & $77.14$ & $\bf 78.40$ & $78.12$ & \textcolor{blue}{$\bf 79.19$} \\
Dev & $50.8$ & $67.40$ & $74.90$ & $-$ & $77.14$ & $\bf 78.40$ & $78.07$ & \textcolor{blue}{$\bf 79.12$} \\
%Test-P & $51.4$ & $67.00$ & $74.50$ & $78.87$ & $77.87$ & $\bf 79.50$ & $78.18$ & \textcolor{blue}{$\bf 79.96$} \\ 
%Test-P & $51.4$ & $67.00$ & $74.50$ & $78.87$ & $77.87$ & $\bf 79.50$ & $78.36$ & \textcolor{blue}{$\bf 80.05$} \\ % arXiv
Test-P & $51.4$ & $67.00$ & $74.50$ & $78.87$ & $77.87$ & $\bf 79.50$ & $78.36$ & \textcolor{blue}{$\bf 80.37$} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

Since \short{} only handles one image and one text input at pre-training, the ‘modality embedding’ is extended to help distinguish the additional image presented in the NLVR2 task. For the Triplet setup, we concatenate the image regions and then feed into the UNITER model. An MLP transform is applied on the [CLS] output for binary classification. For the Pair setup, we treat one input example as two text-image pairs by repeating the text. The two [CLS] outputs from UNITER are then depth concatenated as the joint embedding for the example. Another MLP further transform this embedding for the final classification. For the Pair-biattn setup, the input format is the same as the Pair setup. As for the joint representation, instead of rely on only two [CLS] outputs, we apply a multi-head attention layer (Vaswani et al., 2017) on one sequence of joint image-text embeddings to attend to the other sequence of embeddings, and vice versa.


on the public leaderbaord. Our 3.2% accuracy gain over the SotA GQA method is higher than VQA, possibly because GQA requires more visual reasoning. Thus our framework, with novel encoders and cross-modality pre-training, is suitable and achieves a 4.6\% improvement on opendomain questions (‘Open’ in Table 2)
Results are presented in Table~\ref{tab:gqa_result}.  blabla...

\begin{table*}[h]
\begin{center}
\scriptsize
\caption{Evaluation results on GQA.}
\label{tab:gqa_result}
\begin{tabular}{l|cccc|>{\columncolor[gray]{0.90}}c>{\columncolor[gray]{0.90}}c}
\toprule
Method & LXMERT & MMN~\cite{chen2019meta} & 12-in-1 & NSM~\cite{hudson2019learning} & \shortb{} & \shortb$^*$  \\ \midrule
Test-dev & $60.00$ & $-$ & $-$ & $-$ & $61.19$ & $ $\bf 61.58$ $ \\
Test-std & $60.33$ &  $60.83$ & $60.65$ & \textcolor{blue}{$\bf 63.17$} & $61.23$ & $\bf 61.62$\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


\begin{table*}[h]
\begin{center}
\scriptsize
\caption{Evaluation results on GQA.}
\label{tab:gqa_result}
\begin{tabular}{c|cc}
\toprule
Method & Test-dev & Test-std \\ \midrule
LXMERT~\cite{tan2019lxmert} & $60.00$ & $60.33$ \\
MMN~\cite{chen2019meta} & $-$ &  $60.83$  \\
12-in-1~\cite{lu201912} & $-$ &  $60.65$  \\
NSM~\cite{hudson2019learning} & $-$ & \textcolor{blue}{$ 63.17$} \\ \hline
\rowcolor{Gray} 
\shortb{} & $61.19$ & $61.23$ \\
\rowcolor{Gray} 
\shortb$^*$ &  ${\bf 61.58}$ & ${\bf 61.62}$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}
